Plausibility Is Not Prediction: Contrastive Evidence for LLM-Based Cellular Perturbation Reasoning

Perturbation experiments are central to understanding cellular mechanisms, but remain costly and sparse, motivating prediction of gene expression responses for unobserved conditions. A promising recent direction leverages large language models (LLMs) as "virtual cell" simulators-using stepwise, knowledge-grounded mechanistic reasoning to infer differential expression-pointing toward an interpretable, knowledge-driven paradigm that transcends purely data-driven approaches. However, we find that plausibility is not prediction: despite producing biologically plausible explanations, these methods fail to capture perturbation-specific effects: systematically overestimating differential expression, often underperforming a simple gene-frequency baseline in aggregate evaluations, and collapsing to chance-level performance at the per-gene level. This reveals a reliance on intrinsic gene response tendencies rather than true perturbation reasoning. We trace this failure to how evidence is presented: existing methods evaluate perturbation-gene pairs in isolation, without exposing how related perturbations differ in their effects on the same gene. To address this limitation, we introduce CORE (Contrastive Organization of Relational Evidence), which reframes prediction as a comparison task by organizing evidence into positive and negative outcomes from related perturbations. Using a biomedical knowledge graph for evidence retrieval, CORE improves calibration and substantially boosts perturbation-specific prediction in both LLM-based and non-LLM settings: for example, on drug-perturbation data, CORE-Reasoning improves Qwen3.5-9B aggregate metrics by up to 28.6%, while on generic perturbation data, CORE-Voting raises macro-per-gene AUROC from chance to 0.703 in average across four cell lines. This highlights contrastive evidence organization as essential to reliable LLM-based perturbation reasoning

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction state the paper's main diagnostic claim that biologically plausible LLM reasoning is not sufficient for perturbation-specific prediction, and introduce CORE as a contrastive evidence-organization framework. The corresponding evidence is provided in the motivation, method, and experiment sections, with dataset, knowledge-graph, prompt, inference, and metric details in Appendices~\ref{app:dataset-details}--\ref{app:experimental-details}. The stated scope is limited to binary differential-expression prediction in the evaluated fixed-cell-context settings.


\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations and broader-impact section states that the study is restricted to binary differential-expression prediction in fixed cellular contexts, leaving dose, time, protocol variation, expression magnitude, and uncertainty in DEG calling for future work. Appendices~\ref{app:kg-resources}--\ref{app:method-details} further discuss KG endpoint coverage, missing KG evidence, disconnected or unmapped perturbations, and weak name-based fallback; Appendix~\ref{app:case-study} analyzes failure cases where CORE-Reasoning can be confidently wrong under weak mapping or sparse evidence.


\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not present formal theoretical results or proof-based claims. The mathematical content defines the support setting, gene-prior baseline, CORE evidence aggregation, similarity weighting, and anchor smoothing used by the method.


\item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper specifies the task setup, perturbation-disjoint support/test protocol, C32 and K562 dataset construction, KG harmonization, CORE scoring procedure, prompt serialization, LLM inference protocol, output parsing, and evaluation metrics in the method and experiment sections and Appendices~\ref{app:dataset-details}--\ref{app:experimental-details}. These details cover the experimental components that support the main claims; the separate question below addresses whether code and processed data are released.


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We used the public datasets and KG resouces, and stated their sources explicitly in our paper. We will release all data and code upon paper acceptance. Therefore, we answer "No" as we do not provide anonymized code repository.

\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix~\ref{app:dataset-details} gives dataset preprocessing, DEG labeling, perturbation-disjoint train/test splits, support budgets, and dataset statistics. Appendices~\ref{app:kg-resources}--\ref{app:experimental-details} specify KG construction and coverage, CORE evidence construction, voting weights, fallback mapping, prompt design, LLM inference settings, output parsing, and evaluation metrics. The main methods are deterministic or inference-time prompting methods, so no optimizer-based training is used for the reported CORE-Voting or CORE-Reasoning results.


\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We report matched benchmark metrics, support-budget sweeps, calibration statistics, per-gene metrics, and full numerical tables, but we do not report confidence intervals, error bars, repeated-run statistics, or formal significance tests for the main quantitative comparisons.

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix E.1 reports several inference settings, including the SGLang backend, tensor parallel size, memory fraction, maximum context length, batch size, and one-GPU shard execution. However, we do not yet provide the GPU type, wall-clock runtime, storage requirements, or total compute required for the main experiments.

\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The work uses existing perturbation datasets, public biomedical knowledge resources, and LLM inference for scientific prediction and analysis. It does not involve new human-subject experiments, private individual-level data collection, deception, or deployment of a decision system affecting individuals.

\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations and broader-impact section discusses potential positive impacts, including more auditable LLM-assisted perturbation reasoning and experimental hypothesis prioritization. It also discusses risks from over-reliance on model predictions, stating that CORE outputs should not replace expert review, experimental validation, or clinical decision-making.


\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release a high-risk generative model, scraped media dataset, or private biological dataset. CORE is an evidence-organization and evaluation framework built on existing perturbation data, biomedical KGs, and LLM prompting, so the high-risk release safeguards described in this checklist item are not directly applicable.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We cite and describes the main existing assets used in the experiments, including perturbation datasets, VCWorld-style baselines, public biomedical KG sources, the LLM checkpoint, and inference infrastructure. However, it does not yet explicitly list the licenses or terms of use for these assets, including C32/PerturbQA data, VCWorld, PrimeKG, HetioNet, PertKGE, BioKG, Qwen, and SGLang.

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We introduce ReasonKG (a knowledge graph constructed from multiple public biomedical knowledge graphs) and CORE evidence packets, and Appendix C documents the graph sources, harmonization procedure, node/relation statistics, coverage, and missing-evidence handling. We will release all with license and usage instructions upon acceptance, including ReasonKG, processed evidence packets, prompts, code, and metadata.

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing experiments or new research with human subjects. It uses existing perturbation datasets, benchmark labels, biomedical KG resources, and LLM inference.

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The work does not involve study participants, crowdsourcing, or new human-subject data collection. Therefore IRB approval or equivalent participant-risk disclosure is not applicable.

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLM usage is an important component of the research: the paper evaluates VCWorld- and SUMMER-style LLM perturbation reasoning baselines and introduces CORE-Reasoning, which serializes contrastive same-gene evidence and KG paths into structured prompts for LLM prediction. Section~\ref{sec:method-core-reasoning} and Appendix~\ref{app:llm-inference-protocol} describe the LLM evidence packet, prompt output contract, inference backend, decoding settings, and parsing procedure.


\end{enumerate}
